Bosonic Contribution to Parity-Violating M{\o}ller Scattering at NNLO

We calculate the dominant bosonic two-loop virtual electroweak corrections to parity-violating M{\o}ller scattering at low energies. The electron effective weak charge is extracted from the polarization asymmetry, retaining all contributions that are enhanced by $(1-4\sin^2\theta_W)^{-1}$ or $\ln^2(M_{W,Z}^2/Q^2)$ relative to the tree-level contribution. Analytical results are obtained using the expansion by regions method in the low-energy limit $Q^2\ll M_{W,Z}^2$. Within this approximation, the dominant two-loop bosonic corrections shift the electron effective weak charge (or equivalently the polarization asymmetry) by $0.3\%$. We examine the origin of the leading contributions to this result and assess the remaining theoretical uncertainty from purely bosonic contributions for the MOLLER experiment to about 0.1%.

==> defs.tex <==
% hyphenation patterns
\hyphenation{brems-strah-lung coun-ter-terms La-gran-gi-an}

%  Abbreviations and math space and characters
\RequirePackage{xspace}
\providecommand*\eg{e.g.\@\xspace}
\providecommand*\ie{i.e.\@\xspace}
\providecommand*\cf{cf.\@\xspace}
\providecommand*\etc{etc.\@\xspace}
\providecommand*\etal{et al.\@\xspace}

% roman letters for mathematical constants and operators
\providecommand{\rd}{\ensuremath{\mathrm{d}}}
\providecommand{\re}{\ensuremath{\mathrm{e}}}
\providecommand{\rE}{\ensuremath{\mathrm{E}}}
\providecommand{\ri}{\ensuremath{\mathrm{i}}}
\renewcommand{\Re}{\mathop{\mathrm{Re}}\nolimits}
\renewcommand{\Im}{\mathop{\mathrm{Im}}\nolimits}
\newcommand{\Tr}{\mathop{\mathrm{Tr}}\nolimits}
\providecommand{\hc}{\ensuremath{\text{h.c.}}\xspace}

% mathematical objects 
%\newcommand{\order}[1]{\ensuremath{\mathcal{O}{\left(#1\right)}}\xspace}
\newcommand{\order}[1]{\ensuremath{\mathcal{O}{(#1)}}\xspace}
\let\gsim\gtrsim
\let\lsim\lesssim
\makeatletter
\def\asymp#1%
{\mathrel{\raisebox{-.4em}{$\widetilde{\scriptstyle #1}$}}}
%\newcommand{\dsl}[1]{\not \hspace{-0.7mm}#1}
\def\Nlim#1{\mathrel{\raisebox{-.4em}
{$\stackrel{\displaystyle\longrightarrow}{\scriptstyle#1}$}}}
\def\dsl{\mathpalette\make@slash}
\def\make@slash#1#2{\setbox\z@\hbox{$#1#2$}%
  \hbox to 0pt{\hss$#1/$\hss\kern-\wd0}\box0}
\makeatother
\DeclareMathOperator{\sgn}{sgn}
\newcommand{\sumbar}{\mathop{\overline{\sum}}}

% new commands for cross referencing
\def\refeq#1{\mbox{(\ref{#1})}}
\def\reffi#1{\mbox{Figure~\ref{#1}}}
\def\reffis#1{\mbox{Figures~\ref{#1}}}
\def\refta#1{\mbox{Table~\ref{#1}}}
\def\reftas#1{\mbox{Tables~\ref{#1}}}
\def\refse#1{\mbox{Section~\ref{#1}}}
\def\refses#1{\mbox{Sections~\ref{#1}}}
\def\refapp#1{\mbox{App.~\ref{#1}}}
\def\reffi#1{\mbox{Fig.~\ref{#1}}}
\def\reffis#1{\mbox{Figs.~\ref{#1}}}
\def\refta#1{\mbox{Table~\ref{#1}}}
\def\reftas#1{\mbox{Tables~\ref{#1}}}
\def\refse#1{\mbox{Section~\ref{#1}}}
\def\refses#1{\mbox{Sections~\ref{#1}}}
\def\refapp#1{\mbox{App.~\ref{#1}}}
\def\refapps#1{\mbox{Apps.~\ref{#1}}}
\def\citere#1{\mbox{Ref.~\cite{#1}}}
\def\citeres#1{\mbox{Refs.~\cite{#1}}}

\def\nn{\nonumber}

% shorthand for environments
\newcommand\nl{\notag\\}
\newcommand*\beq{\begin{equation}}
\newcommand*\eeq{\end{equation}}
\newcommand*\beqar{\begin{eqnarray}}
\newcommand*\eeqar{\end{eqnarray}}
\newcommand*\barr{\begin{array}}
\newcommand*\earr{\end{array}}
\newcommand*\bfi{\begin{figure}}
\newcommand*\efi{\end{figure}}
\newcommand*\btab{\begin{table}}
\newcommand*\etab{\end{table}}
\newcommand*\bpm{\begin{pmatrix}}
\newcommand*\epm{\end{pmatrix}}

%Shorthands for Greek letters
\newcommand{\al}{\alpha}
\newcommand{\be}{\beta}
\newcommand{\ga}{\gamma}
\newcommand{\de}{\delta}
\newcommand\eps{\epsilon}
\newcommand\veps{\varepsilon}
\newcommand\la{\lambda}
\newcommand\om{\omega}
%\newcommand{\si}{\sigma}
\newcommand{\De}{\Delta}
\newcommand{\Ga}{\Gamma}
\newcommand\La{\Lambda}
\newcommand{\Si}{\Sigma}

% Units
\providecommand*\USP{\,}
\newcommand*{\Unit}[2]{\ensuremath{#1\USP\text{#2}}}
\newcommand{\pba}{\unskip\,\mathrm{pb}}
\newcommand{\fb}{{\ensuremath\unskip\USP\text{fb}}\xspace}
\newcommand{\MeV}{\ensuremath{\unskip\USP\text{Me\kern -0.1em V}}\xspace}
\newcommand{\GeV}{\ensuremath{\unskip\USP\text{Ge\kern -0.1em V}}\xspace}
\newcommand{\TeV}{\ensuremath{\unskip\USP\text{Te\kern -0.1em V}}\xspace}

% delta function
\newcommand{\deuf}{{\de^{(4)}}}

% SM parameters
\newcommand{\GF}{\ensuremath{G_\mu}}
\newcommand{\rs}{{\mathrm{s}}}
\newcommand{\rw}{{\mathrm{w}}}
\newcommand{\sw}{s_W}
\newcommand{\cw}{c_W}
\newcommand{\sweff}{s_{\mathrm{eff},\ell}}
\newcommand{\gs}{\ensuremath{g_\mathrm{s}}\xspace}
\newcommand{\alphas}{\ensuremath{\alpha_\rs}\xspace}
\newcommand{\Dalphahad}{\ensuremath{\Delta\alpha^{(5)}_{\mathrm{had}}\xspace}}
\newcommand{\If}{\ensuremath {I_{\rw,\Pf}^3}}
\newcommand{\Qf}{\ensuremath {Q_\Pf}}
\newcommand{\Qq}{\ensuremath {Q_\Pq}}
\newcommand{\Ql}{\ensuremath {Q_\Pl}}
\newcommand{\Qt}{\ensuremath {Q_\Pt}}
\newcommand{\VKM}{\ensuremath {{V}}}
\newcommand{\CL}{C_{\rL}}
\newcommand{\CR}{C_{\rR}}
\newcommand{\NCf}{\mathswitch {N_{\mathrm{C}}^\Pf}}
\newcommand{\NCt}{\mathswitch {N_{\mathrm{C}}^\Pt}}
\newcommand{\NCl}{\mathswitch {N_{\mathrm{C}}^\Pl}}
\newcommand{\NCq}{\mathswitch {N_{\mathrm{C}}^\Pq}}
\newcommand{\alphams}{\hat{\alpha}}
\newcommand{\Zms}{\hat{Z}}
\newcommand{\ems}{\hat{e}}
\newcommand{\gms}{\hat{g}}
\newcommand{\swms}{\hat{s}_{\rw}}
\newcommand{\cwms}{\hat{c}_{\rw}}
\newcommand{\kappams}{\hat{\kappa}}

% Particles
\newcommand{\Pg}{\ensuremath{\mathrm{g}}\xspace}
\newcommand{\PA}{\ensuremath{\gamma}\xspace}
\newcommand{\PW}{\ensuremath{\text{W}}\xspace}
\newcommand{\PWp}{\ensuremath{\PW^+}\xspace}
\newcommand{\PWm}{\ensuremath{\PW^-}\xspace}
\newcommand{\PWpm}{\ensuremath{\PW^\pm}\xspace}
\newcommand{\PZ}{\ensuremath{\text{Z}}\xspace}
\newcommand{\PH}{\ensuremath{\text{H}}\xspace}
\newcommand{\Pe}{\ensuremath{\text{e}}\xspace}
\newcommand{\Pep}{\ensuremath{\Pe^+}\xspace}
\newcommand{\Pem}{\ensuremath{\Pe^-}\xspace}
\newcommand{\Pm}{\ensuremath{\mu}\xspace}
\newcommand{\Pb}{\ensuremath{\text{b}}\xspace}
\newcommand{\Pt}{\ensuremath{\text{t}}\xspace}
\newcommand{\Pu}{\ensuremath{\text{u}}\xspace}
\newcommand{\Pd}{\ensuremath{\text{d}}\xspace}
\newcommand{\Ps}{\ensuremath{\text{s}}\xspace}
\newcommand{\Pc}{\ensuremath{\text{c}}\xspace}
\newcommand{\Pbj}{\ensuremath{\text{j_b}}\xspace}
\newcommand{\Pj}{\ensuremath{\text{j}}\xspace}
\newcommand{\Pp}{\ensuremath{\text{p}}\xspace}
\newcommand{\Pq}{\ensuremath{q}\xspace}
\newcommand{\Pl}{\ensuremath{l}\xspace}
\newcommand{\Pn}{\ensuremath{\nu}\xspace}
\newcommand{\Pne}{\ensuremath{\nu_{\Pe}}\xspace}
\newcommand{\Pf}{\ensuremath{f}\xspace}
           
% Particle masses and widths
\def\mathswitch#1{\relax\ifmmode#1\else$#1$\fi}
\newcommand{\MWOS}{\ensuremath{M_{\PW,\text{OS}}}\xspace}
\newcommand{\MZOS}{\ensuremath{M_{\PZ,\text{OS}}}\xspace}
\newcommand{\Ml}{\ensuremath{m_\Pl}\xspace}
\newcommand{\Me}{\ensuremath{m_\Pe}\xspace}
\newcommand{\MW}{\ensuremath{M_\PW}\xspace}
\newcommand{\MZ}{\ensuremath{M_\PZ}\xspace}
\newcommand{\MH}{\ensuremath{M_\PH}\xspace}
\newcommand{\Mt}{\ensuremath{m_\Pt}\xspace}
\newcommand{\Mb}{\ensuremath{m_\Pb}\xspace}
\newcommand{\Mf}{\ensuremath{m_\Pf}\xspace}
\newcommand{\Mq}{\ensuremath{m_\Pq}\xspace}
\newcommand{\MP}{\ensuremath{M_P}\xspace}
\newcommand{\GP}{\ensuremath{\Gamma_P}\xspace}
\newcommand{\MV}{\ensuremath{M_V}\xspace}
\newcommand{\GV}{\ensuremath{\Gamma_V}\xspace}
\newcommand{\MPOS}{\ensuremath{M_{P,\,\OS}}\xspace}
\newcommand{\GPOS}{\ensuremath{\Gamma_{P,\OS}}\xspace}
\newcommand{\MVOS}{\ensuremath{M_{V,\OS}}\xspace}
\newcommand{\GVOS}{\ensuremath{\Gamma_{V,\OS}}\xspace}

% Particle widths
\newcommand{\GWOS}{\ensuremath{\Gamma_\PW^\text{OS}}\xspace}
\newcommand{\GZOS}{\ensuremath{\Gamma_\PZ^\text{OS}}\xspace}
\newcommand{\GZ}{\ensuremath{\Gamma_\PZ}\xspace}
\newcommand{\GW}{\ensuremath{\Gamma_\PW}\xspace}
\newcommand{\GH}{\ensuremath{\Gamma_\PH}\xspace}
\newcommand{\Gt}{\ensuremath{\Gamma_\Pt}\xspace}

\newcommand{\ren}{\mathrm{R}}
\newcommand{\rRe}{\mathop{\widetilde{\mathrm{Re}}}\nolimits}
\newcommand{\muR}{\mu_\mathrm{R}}
\newcommand{\muF}{\mu_\mathrm{F}}
\newcommand{\muIR}{\mu_\mathrm{IR}}
\newcommand{\deltaDR}{\eps}
\newcommand{\DR}{\mathrm{DR}}
\newcommand{\MR}{\mathrm{MR}}

% calligraphic symbols
\newcommand{\cA}{\ensuremath{\mathcal{A}}\xspace}
%\newcommand{\cB}{\ensuremath{\mathcal{B}}\xspace}
\newcommand{\cC}{\ensuremath{\mathcal{C}}\xspace}
\newcommand{\cI}{\ensuremath{\mathcal{I}}\xspace}
\newcommand{\cK}{\ensuremath{\mathcal{K}}\xspace}
\newcommand{\cL}{\ensuremath{\mathcal{L}}\xspace}
\newcommand{\cM}{\ensuremath{\mathcal{M}}\xspace}
\newcommand{\cN}{\ensuremath{\mathcal{N}}\xspace}
\newcommand{\cO}{\ensuremath{\mathcal{O}}\xspace}
\newcommand{\cP}{\ensuremath{\mathcal{P}}\xspace}
\newcommand{\cV}{\ensuremath{\mathcal{V}}\xspace}
\newcommand{\cW}{\ensuremath{\mathcal{W}}\xspace}

\newcommand{\ord}{\mathswitch{{\cal{O}}}}
\newcommand{\Oa}{\mathswitch{{\cal{O}}(\alpha)}}
\newcommand{\Oaa}{\mathswitch{{\cal{O}}(\alpha^2)}}
\newcommand{\Oaaa}{\mathswitch{{\cal{O}}(\alpha^3)}}

% roman symbols
\newcommand{\rc}{\ensuremath{\text{c}}\xspace}
\newcommand{\rT}{\ensuremath{\text{T}}\xspace}
\newcommand{\rL}{\ensuremath{\text{L}}\xspace}
\newcommand{\rR}{\ensuremath{\text{R}}\xspace}
\newcommand{\rS}{\ensuremath{\text{S}}\xspace}
\newcommand{\rA}{\ensuremath{\text{A}}\xspace}
\newcommand{\rV}{\ensuremath{\text{V}}\xspace}
\newcommand{\rr}{\ensuremath{\text{r}}\xspace}
\newcommand{\rl}{\ensuremath{\text{l}}\xspace}
\newcommand{\rB}{\ensuremath{\text{B}}\xspace}
\newcommand{\rI}{\ensuremath{\text{I}}\xspace}

\newcommand{\sv}{\ensuremath{\sl v}}

%acronyms
\newcommand{\OS}{{\mathrm{OS}}}
\newcommand{\SU}{{\mathrm{SU}}}
\newcommand{\U}{{\mathrm{U}}}
\newcommand{\QED}{{\mathrm{QED}}}
\newcommand{\QCD}{{\mathrm{QCD}}}
\newcommand{\GSW}{{\mathrm{GSW}}}
\newcommand{\SM}{SM\xspace}
\newcommand{\THDM}{THDM\xspace}
\newcommand{\HSESM}{HSESM\xspace}
\newcommand{\MSSM}{MSSM\xspace}
\newcommand{\MSbar}{\ensuremath{\overline{{\text{MS}}\xspace}}}
\newcommand{\UV}{{\mathrm{UV}}}
\newcommand{\weak}{{\mathrm{weak}}}
\newcommand{\virt}{{\mathrm{virt}}}
\newcommand{\coll}{{\mathrm{coll}}}
\newcommand{\collCT}{{\textrm{coll-ct}}}
\newcommand{\hard}{{\mathrm{hard}}}
\newcommand{\soft}{{\mathrm{soft}}}
\newcommand{\EPA}{{\mathrm{EPA}}}
\newcommand{\ISR}{{\mathrm{ISR}}}
\newcommand{\FSR}{{\mathrm{FSR}}}
\newcommand{\LL}{{\mathrm{LL}}}
\newcommand{\LO}{{\mathrm{LO}}}
\newcommand{\NLO}{{\mathrm{NLO}}}
\newcommand{\PAx}{{\mathrm{PA}}}
\newcommand{\EW}{{\mathrm{EW}}}
\newcommand{\ew}{{\mathrm{EW}}}
\newcommand{\nf}{{\mathrm{nf}}}
\newcommand{\fact}{{\mathrm{fact}}}
\newcommand{\trunc}{{\mathrm{trunc}}}

%codes
\newcommand{\Collier}{{\sc Collier}\xspace}
\newcommand{\HAWKTwo}{{\sc Hawk~2.0}\xspace}
\newcommand{\Recola}{{\sc Recola}\xspace}
\newcommand{\RecolaTwo}{{\sc Recola2}\xspace}
\newcommand{\Prophecy}{{\sc Prophecy4f}\xspace}
\newcommand{\Openloops}{{\sc OpenLoops}\xspace}
\newcommand{\MGNLO}{{\sc MadGraph5\_aMC@NLO}\xspace}
\newcommand{\Gosam}{{\sc GoSam}\xspace}
\newcommand{\FORM}{{\sc FORM}\xspace}
\newcommand{\NLOX}{{\sc NLOX}\xspace}

%special symbols
\newcommand{\gZbox}{\ensuremath{\mathop{\Box}\nolimits_{\gamma Z}}}
\newcommand{\WWbox}{\ensuremath{\mathop{\Box}\nolimits_{WW}}}
\newcommand{\ZZbox}{\ensuremath{\mathop{\Box}\nolimits_{ZZ}}}
% SMEFT parameters
\newcommand{\Lop}{\mathcal{O}}
\newcommand{\Lcoeff}{C}

% new environments
\newenvironment{myenumerate}%
{\begin{enumerate}[label=(\alph*),leftmargin=!,labelindent=0pt,labelwidth=2.5ex,%
   labelsep=.7ex,topsep=2pt plus 1pt minus 1pt,itemsep=2pt plus 1pt minus 1pt,parsep=0pt]}%
{\end{enumerate}}
\newenvironment{myitemize}%
{\begin{itemize}[leftmargin=!,labelindent=0pt,labelwidth=2.5ex,%
   labelsep=.7ex,topsep=2pt plus 1pt minus 1pt,itemsep=2pt plus 1pt minus 1pt,parsep=0pt]}%
{\end{itemize}}
\newenvironment{myaitemize}%
{\begin{itemize}[leftmargin=!,labelindent=0pt,labelwidth=2.5ex,%
   labelsep=.7ex,topsep=2pt plus 1pt minus 1pt,itemsep=4pt plus 2pt minus 2pt,parsep=0pt]}%
{\end{itemize}}

% new paragraph
\makeatletter
\newcommand\myparagraph{\@startsection{paragraph}{4}{\z@}%
  {-10\p@ \@plus 6\p@ \@minus 3\p@}%
  {3\p@}%
  {\normalfont\itshape}%
}
\makeatother

\newcommand*{\doi}[1]{\href{http://dx.doi.org/#1}{doi: #1}}



